Active Measure Reinforcement Learning for Observation Cost Minimization

Standard reinforcement learning (RL) algorithms assume that the observation of the next state comes instantaneously and at no cost. In a wide variety of sequential decision making tasks ranging from medical treatment to scientific discovery, however, multiple classes of state observations are possible, each of which has an associated cost. We propose the active measure RL framework (Amrl) as an initial solution to this problem where the agent learns to maximize the costed return, which we define as the discounted sum of rewards minus the sum of observation costs. Our empirical evaluation demonstrates that Amrl-Q agents are able to learn a policy and state estimator in parallel during online training. During training the agent naturally shifts from its reliance on costly measurements of the environment to its state estimator in order to increase its reward. It does this without harm to the learned policy. Our results show that the Amrl-Q agent learns at a rate similar to standard Q-learning and Dyna-Q. Critically, by utilizing an active strategy, Amrl-Q achieves a higher costed return.

==> library.tex <==
@article{watkins1992,
  title={Q-learning},
  author={Watkins, Christopher JCH and Dayan, Peter},
  journal={Machine learning},
  volume={8},
  number={3-4},
  pages={279--292},
  year={1992},
  publisher={Springer}
}
@inproceedings{chen2017double,
  title={Double-task deep q-learning with multiple views},
  author={Chen, Jun and Bai, Tingzhu and Huang, Xiangsheng and Guo, Xian and Yang, Jianing and Yao, Yuxing},
  booktitle={Proceedings of the IEEE International Conference on Computer Vision Workshops},
  pages={1050--1058},
  year={2017}
}
@book{powell2007approximate,
  title={Approximate Dynamic Programming: Solving the curses of dimensionality},
  author={Powell, Warren B},
  volume={703},
  year={2007},
  publisher={John Wiley \& Sons}
}
@inproceedings{li2019multi,
  title={Multi-View Reinforcement Learning},
  author={Li, Minne and Wu, Lisheng and Jun, WANG and Ammar, Haitham Bou},
  booktitle={Advances in Neural Information Processing Systems},
  pages={1418--1429},
  year={2019}
}
@article{mnih2015human,
  title={Human-level control through deep reinforcement learning},
  author={Mnih, Volodymyr and others},
  journal={Nature},
  volume={518},
  number={7540},
  pages={529},
  year={2015},
  publisher={Nature Publishing Group}
}
@article{kaelbling1998planning,
  title={Planning and acting in partially observable stochastic domains},
  author={Kaelbling, Leslie Pack and Littman, Michael L and Cassandra, Anthony R},
  journal={Artificial intelligence},
  volume={101},
  number={1-2},
  pages={99--134},
  year={1998},
  publisher={Elsevier}
}
@inbook{gibson1966senses,
  title={The senses considered as perceptual systems.},
  author={Gibson, James Jerome},
  year={1966},
  publisher={Houghton Mifflin}
}
@article{bossens2019learning,
  title={Learning to learn with active adaptive perception},
  author={Bossens, DM and Townsend, Nicholas C and Sobey, AJ},
  journal={Neural Networks},
  volume={115},
  pages={30--49},
  year={2019},
  publisher={Elsevier}
}
@misc{brockman2016openai,
    title={OpenAI Gym},
    author={Greg Brockman and Vicki Cheung and Ludwig Pettersson and Jonas Schneider and John Schulman and Jie Tang and Wojciech Zaremba},
    year={2016},
    eprint={1606.01540},
    archivePrefix={arXiv},
    primaryClass={cs.LG}
}
@inproceedings{akrour2012april,
  title={April: Active preference learning-based reinforcement learning},
  author={Akrour, Riad and Schoenauer, Marc and Sebag, Mich{\`e}le},
  booktitle={Joint European Conference on Machine Learning and Knowledge Discovery in Databases},
  pages={116--131},
  year={2012},
  organization={Springer}
}
@article{dietterich2000hierarchical,
  title={Hierarchical reinforcement learning with the MAXQ value function decomposition},
  author={Dietterich, Thomas G},
  journal={Journal of artificial intelligence research},
  volume={13},
  pages={227--303},
  year={2000}
}
%model-based RL
@inproceedings{sutton1990,
  title={Integrated architectures for learning, planning, and reacting based on approximating dynamic programming},
  author={Sutton, Richard S},
  booktitle={Machine learning proceedings 1990},
  pages={216--224},
  year={1990},
  publisher={Elsevier}
}

@inproceedings{kumar2016optimal,
  title={Optimal control with learned local models: Application to dexterous manipulation},
  author={Kumar, Vikash and Todorov, Emanuel and Levine, Sergey},
  booktitle={2016 IEEE International Conference on Robotics and Automation (ICRA)},
  pages={378--383},
  year={2016},
  organization={IEEE}
}
@inproceedings{levine2013guided,
  title={Guided policy search},
  author={Levine, Sergey and Koltun, Vladlen},
  booktitle={International Conference on Machine Learning},
  pages={1--9},
  year={2013}
}
@inproceedings{deisenroth2011pilco,
  title={PILCO: A model-based and data-efficient approach to policy search},
  author={Deisenroth, Marc and Rasmussen, Carl E},
  booktitle={Proceedings of the 28th International Conference on machine learning (ICML-11)},
  pages={465--472},
  year={2011}
}
@inproceedings{gal2016improving,
  title={Improving PILCO with Bayesian neural network dynamics models},
  author={Gal, Yarin and McAllister, Rowan and Rasmussen, Carl Edward},
  booktitle={Data-Efficient Machine Learning workshop, ICML},
  volume={4},
  pages={34},
  year={2016}
}
%active RL
@article{Settles2012,
    title={Active learning},
  author={Settles, B.},
  journal={ Synthesis Lectures on Artificial Intelligence and Machine Learning},
  pages={1--114},
  year={2012},
  publisher={Elsevier}
}

@inproceedings{epshteyn2008active,
  title={Active reinforcement learning},
  author={Epshteyn, Arkady and Vogel, Adam and DeJong, Gerald},
  booktitle={Proceedings of the 25th international conference on Machine learning},
  pages={296--303},
  year={2008}
}
@inproceedings{krueger2016active,
  title={Active reinforcement learning: Observing rewards at a cost},
  author={Krueger, David and Leike, Jan and Evans, Owain and Salvatier, John},
  booktitle={Future of Interactive Learning Machines, NIPS Workshop},
  year={2016}
}

@inproceedings{lopes2009active,
  title={Active learning for reward estimation in inverse reinforcement learning},
  author={Lopes, Manuel and Melo, Francisco and Montesano, Luis},
  booktitle={Joint European Conference on Machine Learning and Knowledge Discovery in Databases},
  pages={31--46},
  year={2009},
  organization={Springer}
}
@inproceedings{doshi2008reinforcement,
  title={Reinforcement learning with limited reinforcement: Using Bayes risk for active learning in POMDPs},
  author={Doshi, Finale and Pineau, Joelle and Roy, Nicholas},
  booktitle={Proceedings of the 25th international conference on Machine learning},
  pages={256--263},
  year={2008}
}
@article{schulze2018active,
  title={Active reinforcement learning with monte-carlo tree search},
  author={Schulze, Sebastian and Evans, Owain},
  journal={arXiv preprint arXiv:1803.04926},
  year={2018}
}
@article{thalken2005synthesis,
  title={Synthesis for semiconductor device design},
  author={Thalken, Jason and Haas, Stephan and Levi, AFJ},
  journal={Journal of applied physics},
  volume={98},
  number={4},
  pages={044508},
  year={2005},
  publisher={American Institute of Physics}
}
